Data-driven Reference Trajectory Optimization for Precision Motion Systems

We propose a data-driven optimization-based pre-compensation method to improve the contour tracking performance of precision motion stages by modifying the reference trajectory and without modifying any built-in low-level controllers. The position of the precision motion stage is predicted with data-driven models, a linear low-fidelity model is used to optimize traversal time, by changing the path velocity and acceleration profiles then a non-linear high-fidelity model is used to refine the previously found time-optimal solution. We experimentally demonstrate that the proposed method is capable of simultaneously improving the productivity and accuracy of a high precision motion stage. Given the data-based nature of the models, the proposed method can easily be adapted to a wide family of precision motion systems.

==> data/percent_improvement.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
$\mathtt{a_{max}}$ $(\mathrm{m~s^{-2}$	&Shape	&time (s)	&$L_1$	&$L_2$	&$L_\infty$\\
\toprule
				&Letter u	&1.0517	&212\%	&250\%	&270\%	\\
				&Letter r	&0.8075	&243\%	&280\%	&401\%	\\
1				&Letter c	&0.8073	&501\%	&464\%	&390\%	\\
				&Letter h	&0.9711	&136\%	&149\%	&145\%	\\ 
				&\Airfoil	&1.3222	&378\%	&322\%	&285\%	\\
\midrule
				&Letter u	&0.7483	&177\%	&187\%	&220\%	\\
				&Letter r	&0.5741	&153\%	&164\%	&188\%	\\
2				&Letter c	&0.574	&234\%	&231\%	&303\%	\\
				&Letter h	&0.6904	&143\%	&164\%	&279\%	\\
				&\Airfoil	&1.0837	&469\%	&423\%	&581\%	\\
\midrule
				&Letter u	&0.6183	&157\%	&163\%	&186\%	\\
				&Letter r	&0.4731	&149\%	&142\%	&175\%	\\
3				&Letter c	&0.4733	&167\%	&163\%	&219\%	\\
				&Letter h	&0.5678	&129\%	&137\%	&176\%	\\
				&\Airfoil	&1.0239	&400\%	&270\%	&139\%


==> data/table_percent_improv.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                                                  %%
%%  This is a LaTeX2e table fragment exported from Gnumeric.        %%
%%                                                                  %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\$$\backslash$mathtt\{a\_\{max\}\}	&Shape	&time (s)	&\$L\_1\$	&\$L\_2\$	&\$L\_\{$\backslash$infty\}\$	&\\
1	&u						&1.052	&52.7	&60.0	&63.0	&\\
	&r						&0.807	&58.9	&64.3	&75.1	&\\
	&c						&0.807	&80.0	&78.5	&74.4	&\\
	&h						&0.971	&26.6	&32.8	&31.0	&\\
	&$\backslash$airfoil	&1.322	&73.5	&69.0	&64.9	&\\
3	&u						&0.618	&36.4	&38.7	&46.1	&\\
	&r						&0.473	&32.8	&29.7	&42.9	&\\
	&c						&0.473	&40.2	&38.6	&54.3	&\\
	&h						&0.568	&22.6	&27.0	&43.1	&\\
	&$\backslash$airfoil	&1.024	&75.0	&63.0	&28.1	&\\


==> old/3-data_driven_modelling__conflicted_copy_2022-03-22_162423_.tex <==
%Give an overview of the model types.
%As we take the machine to be a black-box, the method proposed in this paper relies exclusively on models identified from experimental data. In practice, we input trajectories and obtain measurements as time-series data and assume that the sampling rate is high enough to capture the system dynamics.

As a first approximation, we model the system using a continuous-time linear model which captures the dominant dynamics. The structure of this model allows for efficient computations of a time-optimal solution in the first stage, but lacks the high-precision required by the application. This shortcoming is alleviated by a second high-fidelity neural network model, used for refining the initial guess provided by the lower-fidelity linear model.

%\dlm{\emph{A key thing to keep is mind is were trying to sell this as a methodology that can be used to improve any machine. This means that things should be written as if they're being applied to a ``abstract'' machine, rather than too our specific experimental setup}}.
%\subsubsection{Experimental Design/Data-set overview}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Training data data generation}
Choosing input trajectories that cover a wide range of operational regions is essential for generating informative data to train models that can generalize to previously unseen trajectories. Classical system identification methods make use of a toolbox of excitation signals such as Pseudo Random Binary Signal (PRBS), sinusoidal, or chirp signals. These inputs have the property of being persistently exciting for linear systems. Unfortunately none of these proved adequate for the identification of the nonlinear system in this paper. 
%
Most machines, including the experimental setup described in Section~\ref{subsec:setup}, impose velocity and acceleration limits on input trajectories to prevent damage to the system. PRBS signals contain discontinuities that trigger these safety checks and are thus unsuitable for our purposes. Sinusoidal and chirp signals also proved inadequate for our purposes, as they excited modes of our experimental apparatus that are not relevant for our problem, in particular low frequency oscillations between the machine and supporting structure. 

For the identification of both the linear and nonlinear models we opted to instead use randomly generated trajectories with varying geometry and acceleration. We generate a large number of trajectories (containing a total of approximately $10^{7}$ data points) by randomly changing the velocity, acceleration, or jerk of the input trajectory at random times subject to the operational limits of the machine. The resulting trajectories are rich in features seen on real parts, for example curves of different radii, traversed at different speeds and appearing in different locations within the workspace, as well as sharp transitions in acceleration and jerk. They are not designed for a specific part, but for a particular set of constraints on velocity and acceleration. A representative training data sample is shown in Figure~\ref{fig:xy-training-data}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Low-fidelity linear model} \label{sec:linear-model}
%We use the low-fidelity model to make a trade-off between speed and precision. Our goal when constructing the model is to capture the fundamental low-frequency dynamics of the machine.

The closed-loop system maps trajectories to trajectories and is of the form $\gamma = F(\rho)$. We approximate this mapping using a linear time invariant (LTI) state space model of the following form
\begin{subequations} \label{eq:linearmodel}
	\begin{align}
		\dot x(t) &= A x(t) + B \ReferenceOne(t) \mathrm {,} \label{eq:linearmodel-a}\\
		\OutputOne(t) &= C x(t) + D \ReferenceOne(t) \mathrm{.} \label{eq:linearmodel-b}
	\end{align}
\end{subequations}
The model \eqref{eq:linearmodel} uses a non-physical hidden state $x \in \reals^4$; the matrices $A$, $B$, $C$, and $D$ are identified from experimental data using the \verb|MATLAB| function \verb|n4sid| from the system identification toolbox.

%The linear model was evaluated in the \Letters~test set, the results are shown in Table \ref{tab:linear-model-acc}. 
The linear model captures the dominant system dynamics (model validation results are presented in Section~\ref{sec:num-results}), allowing us to solve a minimum time problem that effectively trades off precision and accuracy, as described in Section~\ref{sec::stage-one}. However, it fails to capture some of the nonlinearities inherent in the system and is not on its own sufficiently accurate to achieve the precision required by the application. \ar{It is still unclear, what is the purpose of this model - why is it not possible without it? Also, the performance is provided later in the Validation subsection, might be good to mention that . The purpose of it is mentioned in the beginning of the section, and should be re-iterated here.}

% The continuous time linear model can be numerically evalulated in discrete time with a Runge-Kutta method of order 4:

% \begin{subequations}
% 	\begin{align}
% 		x_{k+1}	&= x_{k} + \frac{\DeltatOne_k}{are6}\left(w_1 + 2 w_2 + 2 w_3 + w_4\right)\mathrm {,}\\
% 		t_{k+1}	&= t_k + \DeltatOne_k \mathrm {,}\\
% 		w_1		&= g(x_k, \ReferenceOne_k) \mathrm {,}\\
% 		w_2		&= g(x_k + \frac{\DeltatOne_k}{2}w_1, ?\ReferenceOne_k + ?\ReferenceOne_{k+1}) \mathrm {,}\\ 
% 		w_3		&= g(x_k + \frac{\DeltatOne_k}{2}w_2, ?\ReferenceOne_k + ?\ReferenceOne_{k+1}) \mathrm {,}\\ 
% 		w_4		&= g(x_k + \DeltatOne_k w_3, ?\ReferenceOne_k + ?\ReferenceOne_{k+1}) \mathrm {,}\\
% 		\OutputOne_{k+1} &= C x_{k+1} + D \ReferenceOne_{k+1} \mathrm {.}
% 	\end{align}
% \end{subequations}

% \begin{itemize}
% 	%\item Training data
%     %\item Approach from SysID
%     \item Validation metrics (least squares fit RMS error?)
% \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{High-fidelity Nonlinear Model} \label{sec:nonlinear-model}

To obtain a higher precision model, we chose to use a neural network (NN) to capture the nonlinearities of the system dynamics.
NN are significantly more expressive than linear models, but require more informative training data to avoid overfitting.
We also considered other alternatives such as Gaussian Processes, but found that the NN architecture below offered a more favourable trade-off between accuracy and computation.
They are suited for our application, where a large amount of data can be collected at low cost.
%However more informative training data is needed and the possibility of overfitting needs to be carefully addressed. 
%
%\dlm{This paragraph is a bit weak, maybe a better comment would be that GPs become very expensive as more data is added, given how much data we use, I assume a even evaluating a GP would be insanely expensive} \td{$\Leftarrow$ Partially addressed}
%
%Other alternatives were considered, in particular Gaussian Processes (GP). The amount of data required to obtain a good representation of the system would make evaluations of a GP model prohibitely expensive. That made us opt for the more scalable NN.

The 2D-positioning stage is modelled using two independent causal artificial neural networks, one for each axis. The two NNs are structurally identical, but are trained separately, leading to different weights. Each takes as input the most recent $500 \mathrm{m s}$ of the reference for the corresponding axis, subsampled at $400 \mathrm{Hz}$, leading to $200$ inputs. Each network has a single output, namely the predicted position at the subsequent time step. The networks have $8$ fully connected hidden layers of LeakyReLU activation functions with a slope of $0.01$, and a triangular structure as illustrated in Figure~\ref{fig:nn}.
%
The choice of feed-forward (as opposed to recurrent) NN was made to ensure that the model prediction accuracy does not degrade over time due to compounding errors. We note also that by training separate NN for each axis we are implicitly ignoring coupling effects between the two axis; this choice is supported by experimental data that suggests that this effect is negligible, as demonstrated in Section~\ref{sec:num-results}.
%Only input information is used to predict an output point, i.e., the network is not recurrent. This approach ensures that the model prediction accuracy cannot degrade over time due to compounding errors as might occur when using e.g., a recurrent NN. This model structure also doesn't capture coupling effects between the two axis. However, this effect is negligible and the prediction accuracy with this structure is adequate for our purposes as demonstrated in Section~\ref{sec:num-results}.
%
Finally, note that the nonlinear and linear models are independent, in particular the predicitions of the linear model are not used in the nonlinear model evaluation.

%The feedforward nature of this network makes predictions of the output only dependent on the reference provided, and not recursively on previous predictions. This has two main advantages: prediction errors do not propagate, and the optimization problem is less coupled and thus easier to solve.
%\td{Elaborate! discuss why and how you chose this structure, tell me why you didn't use a recursive type NN}.


 %The output is a single value predicting the output at the next time step. 
% The nonlinear model represented by the NN aims at achieving a prediction error substancially smaller than the acceptable deviation between output and target geometry.
% Metrics on the performance of the nonlinear model are given in \ref{sec:num-results}.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{img/xy-training-data} %xy
		\caption{Sample of the data collected to train and test the nonlinear neural network model. A total of about $\approx 10^{7}$ data points were collected for this purpose.
			%\todo[inline]{Change labels to $(x_\Output, y_\Output)$, etc.}
			%\todo[inline]{Add frames to $\Objective$}
		}
		\label{fig:xy-training-data}
	\end{center}
\end{figure}


Having sufficient high-quality data is necessary to ensure that the NN is accurate and generalizes well. To train the NN, we augment the random trajectories used to train the linear model (see Section~\ref{sec:linear-model}) with a set of varied regular geometries such as circles, polygons, and spirals. A representative sample of the data used to train the NN is displayed in Figure~\ref{fig:xy-training-data}.
To enrich the data set further, after training the NN with this data the optimisation methodology of Section \ref{sec:approach} was applied to the same regular geometries, the optimised input trajectories were applied to the machine in additional experiments, and the additional data was used to retrain the NN.
%
%In an iterative process, we then apply the optimization methodology from Sections~\ref{sec:stage-one}-\ref{sec:stage-two} to these geometries and add the resulting data to the data set. This process is used to sure that
In this way, solutions of the optimization problem that achieve good performance in simulation
by exploiting spurious features of one generation of the nonlinear model are included in the training of the next generation nonlinear model.
These data sets lead to a targete reduction in overfitting in areas that are favoured by the optimization. Overall, our strategy is to include sufficient random (exploratory) and structured (exploitative) data to ensure the NN is both accurate and generalizes well in the areas of interest.

%\td{The repeatibility of the system is the limiting factor for the precision of the model}

From a total of $\approx 10^7$ experimental data points collected, half for each axis, the data was divided $80\%/20\%$ for training and testing purposes. This results in a ratio of $\approx34$ data points per parameter. About $60\%$ of the data comes from the randomly generated trajectories, and the remaining from regular shapes both before and after optimization. The experimental data is divided in segments of $500~\mathrm{ms}$, subsampled to achieve an effective sample rate of $400\mathrm{Hz}$, and scaled.
For the loss function we use the mean square of the prediction error.
We use batches of $16\mathrm{k}$ segments which take maximum advantage of the GPU computation power. {\it Adam} was used for the optimizer, with decaying learning rate. Modeling and training were done in {\it pytorch} with {\it CUDA} support.

%\td{mention that training details are provided later (or more them here!) It would be really good to emphasize that it was all done using standard tools, this supports our claim that this methodology is easily applicable!}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{neuralnetwork/neuralnetwork} %xy
		\caption{Neural network structure. Each layer is fully connected to the next. The input layer has $200$ neurons, there are $M=8$ hidden layers, with $\{200, 200, 100, 100, 50, 25, 12, 6\}$ neurons, and the output layer has $1$ neuron. The activation function of the hidden layers is a $\mathrm{LeakyReLU}$ function with slope $0.01$, and a bias term. There are total of $117322$ weights to be adjusted in the training. Two independent networks with identical structure were trained, one for each axis.}
			%\todo[inline]{Change labels to $(x_\Output, y_\Output)$, etc.}
			%\todo[inline]{Add frames to $\Objective$}
		\label{fig:nn}
	\end{center}
\end{figure}

%\td{Why is it like this}
%\td{ML best practices: Validation, crossvalidation etc. etc.}

\if 01
Sequential(
  (0): Linear(in_features=200, out_features=200, bias=True)
  (1): LeakyReLU(negative_slope=0.01)
  (2): Linear(in_features=200, out_features=200, bias=True)
  (3): LeakyReLU(negative_slope=0.01)
  (4): Linear(in_features=200, out_features=100, bias=True)
  (5): LeakyReLU(negative_slope=0.01)
  (6): Linear(in_features=100, out_features=100, bias=True)
  (7): LeakyReLU(negative_slope=0.01)
  (8): Linear(in_features=100, out_features=50, bias=True)
  (9): LeakyReLU(negative_slope=0.01)
  (10): Linear(in_features=50, out_features=25, bias=True)
  (11): LeakyReLU(negative_slope=0.01)
  (12): Linear(in_features=25, out_features=12, bias=True)
  (13): LeakyReLU(negative_slope=0.01)
  (14): Linear(in_features=12, out_features=6, bias=True)
  (15): LeakyReLU(negative_slope=0.01)
  (16): Linear(in_features=6, out_features=1, bias=True)
)
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model Validation} \label{sec:num-results}

Our proposed methodology relies heavily on the quality of our data-driven model to improve the performance of the system. In this section, we compare our linear and high-fidelity neural network models with experimental validation data to illustrate the precision we are able to achieve using modern machine learning techniques and best practices.
The quality of the models predictions is evaluated over different datasets and acceleration limits. The results are summarized in Table \ref{tab:linear-model-acc} and Figure \ref{fig:model-hist}.


%\td{Include figure comparing linear, nonlinear, and experimental data as a function of time. Goal is to give the reader a ``typical'' scenario to visualize.} -> r-time (?)

\newcommand{\umph}{}%{~(\mathrm{\mu m})}
\newcommand{\umphb}{\mathrm{\mu m}}
\begingroup
\renewcommand{\arraystretch}{1.3}
\begin{table}
	\begin{center}
		\begin{tabular}{@{}*{8}{r}@{}}
			\toprule
			&&\multicolumn{2}{c}{Training / } 	&\multicolumn{2}{c}{$\mathtt{a_{max}}$} &\multicolumn{2}{c}{$\mathtt{a_{max}}$} \\
			&&\multicolumn{2}{c}{Validation} 	&\multicolumn{2}{c}{$1.0~ \mathrm{m~s^{-2}}$} &\multicolumn{2}{c}{$3.0~ \mathrm{m~s^{-2}}$} \\
			\cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} 			
			Model&Axis	&$\mu\umph$				&$\sigma\umph$  &$\mu\umph$			&$\sigma\umph$			&$\mu\umph$				&$\sigma\umph$\\
			--&--&$\umphb$	&$\umphb$	&$\umphb$	&$\umphb$	&$\umphb$	&$\umphb$	\\
			\midrule 
			Linear		&x		&3.0&48.0		&4.7&30.1	&5.4 &57.2 \\
						&y		&-13.2&156.3	&-0.0&108.5	&0.5&229.4 \\
			\midrule
			Non-linear	&x		&-0.0&3.2		&-0.3&8.2	&1.0&11.1	\\
						&y		&-0.0&6.0		&-2.0&13.4	&-2.3&18.7	\\
			\bottomrule
		\end{tabular}
		\caption{\label{tab:linear-model-acc} Prediction error mean $\mu$ and standard deviation $\sigma$ of the linear and non-linear models. Both models are evaluated in the \Letters~test case, with different maximum acceleleration values $\mathtt{a_{max}}$. The linear model is also evaluated in its training data set, and the non-linear model in its validation data set.}
	\end{center}
\end{table}
\endgroup

\begin{figure}
\centering

\begin{subfigure}{\columnwidth}
	\includegraphics[width = .49\textwidth]{img/hist-data_nosin-a=x0-max_acc=0.0}
	\includegraphics[width = .49\textwidth]{img/hist-data_nosin-a=y-max_acc=0.0}
  \caption{Validation data\label{fig:label1}}
\end{subfigure}\hfill

%\bigskip

\begin{subfigure}{1\columnwidth}
	\includegraphics[width = .49\textwidth]{img/hist-data_letters-a=x0-max_acc=1.0}
	\includegraphics[width = .49\textwidth]{img/hist-data_letters-a=y-max_acc=1.0}
	\caption{\Letters~test case with $\mathtt{a_{max}} \leq 1~\mathrm{m~s^{-2}}$}
  \label{fig:label2}
\end{subfigure}\hfill

%\bigskip

\begin{subfigure}{\columnwidth}
	\includegraphics[width = .49\textwidth]{img/hist-data_letters-a=x0-max_acc=3.0}
	\includegraphics[width = .49\textwidth]{img/hist-data_letters-a=y-max_acc=3.0}
	\caption{\Letters~test case with $\mathtt{a_{max}} \leq 3~\mathrm{m~s^{-2}}$}
  \label{fig:label3}
\end{subfigure}

\caption{Histogram of the prediction error of the non-linear model for its validation dataset and 
	%, i.e. the difference between model predictions and experimental data,
	\Letters~test case with different maximum acceleleration values $\mathtt{a_{max}}$.}
\label{fig:model-hist}

\end{figure}

%\subsection{Model accuracy}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{img/opterror-vs-acc} %xy
		\caption{Prediction error of the nonlinear model as a function of the maximum acceleration $\mathtt{a_{max}}$ of the reference trajectory. The error is evaluated for the letters and airfoil test cases. Above $5~\mathrm{m~s^-2}$ the training data does not contain enough information to train the model properly.
			%\todo[inline]{Change labels to $(x_\Output, y_\Output)$, etc.}
			%\todo[inline]{Add frames to $\Objective$}
		}
		\label{fig:opterror-vs-acc}
	\end{center}
\end{figure}



The linear model training data set includes trajectories with a range of accelerations up to $5~\mathrm{m~s^{-2}}$. However, due to its simple structure, the linear model cannot overfit the data, hence cannot accurately predict all points in its training data set. It performs better when the acceleration is restricted to a lower value, even for trajectories not seen during the fit.

Regarding the nonlinear model, the prediction accuracy is best for data that has the same characteristics as the one used for the training, as can be seen in Figure \ref{fig:label1} where the error is evaluated for the validation dataset. The empirical error distribution has zero mean.
% It is not symmetric. Fisher's moment coefficient of skewness -44 for x, -20 for y axis.
When presented with data coming from shapes which have not been used for the training of the model, the prediction accuracy degrades. However the accuracy is still adequate for the application. The nonlinear model error standard deviations are for all tested geometries below $20~\mathrm{\mu m}$ for each axis for accelerations below $4~\mathrm{m~s^{-2}}$.

Figure \ref{fig:opterror-vs-acc} shows how the standard deviation of the prediction evolves with the maximum acceleration $\mathtt{a_{max}}$ that was set as a constraint. For acceleration values where there is sufficient training data, the model prediction error increase gradually with the acceleration. If we try to use the model outside of the acceleration values it was trained for, the predictions deteriorate.

In this work we set the goal of tracing paths with deviations up to $20~\mathrm{\mu m}$. Although the experimental apparatus can operate at accelerations up to $40~\mathrm{\mu s}$, we are ultimately limited by the model performance to improve the machine precision. For our intended use cases, higher acceleration values, to which corresponds higher model prediction errors are thus not of interest. If they were, training data with higher acceleration content could be collected to train the model in this region.

A representative predicted trajectory from the nonlinear model is shown in Figure~\ref{fig:r-time}, in which the letter ''r`` from the letters test case was simulated by using as reference the target geometry at a constant path speed.
%The simulation matches the experimental data closely.

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=\columnwidth]{img/r-time} %xy
		\caption{The target geometry of the letter ``r'' of the ETH Z\"{u}rich Logo, traveled at a constant path speed of $40\mathrm{mm~s^{-1}}$ is used as the reference. The simulated output corresponds to the prediction of the nonlinear model, which is ploted with the experimental data collected with the same reference. Both simulated and experimental results are compared against the target geometry to compute the deviation. The model predictions follow the experimental data closely. This plot also shows the performance of the built-in tracking controller, with deviations up to $100~\mathrm{\mu m}$.}
			%\todo[inline]{Change labels to $(x_\Output, y_\Output)$, etc.}
			%\todo[inline]{Add frames to $\Objective$}
		\label{fig:r-xy-all}
		\label{fig:r-xy-detail}
	\end{center}
\end{figure}

